Measurement of the double-differential high-mass Drell-Yan cross section in pp collisions at $\sqrt{s}$ = 8 TeV with the ATLAS detector

This paper presents a measurement of the double-differential cross section for the Drell-Yan $Z/\gamma^{*} \rightarrow \ell^{+} \ell^{-}$ and photon-induced $\gamma\gamma \rightarrow \ell^{+} \ell^{-}$ processes where $\ell$ is an electron or muon. The measurement is performed for invariant masses of the lepton pairs, $m_{\ell\ell}$, between 116 GeV and 1500 GeV, using a sample of 20.3 fb$^{-1}$ of pp collisions data at centre-of-mass energy of $\sqrt{s}$ = 8 TeV collected by the ATLAS detector at the LHC in 2012. The data are presented double differentially in invariant mass and absolute dilepton rapidity as well as in invariant mass and absolute pseudorapidity separation of the lepton pair. The single-differential cross section as a function of $m_{\ell\ell}$ is also reported. The electron and muon channel measurements are combined and a total experimental precision of better than 1% is achieved at low $m_{\ell\ell}$. A comparison to next-to-next-to-leading order perturbative QCD predictions using several recent parton distribution functions and including next-to-leading order electroweak effects indicates the potential of the data to constrain parton distribution functions. In particular, a large impact of the data on the photon PDF is demonstrated.

==> Shared/tables/electrons/Correlation_elec_116to150.tex <==
\begin{sidewaystable}[!htb]
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|cccccccccccccccccccccccccc|}
  & $116~\GeV$ & $130~\GeV$ & $0.0$ & $0.2$ & $0.4$ & $0.6$ & $0.8$ & $1.0$ & $1.2$ & $1.4$ & $1.6$ & $1.8$ & $2.0$ & $2.2$ & $0.0$ & $0.25$ & $0.5$ & $0.75$ & $1.0$ & $1.25$ & $1.5$ & $1.75$ & $2.0$ & $2.25$ & $2.5$ & $2.75$\\
 Bin & $< m_{ee}$ & $< m_{ee}$ & $< |y_{ee}|$ & $< |y_{ee}|$ & $< |y_{ee}|$ & $< |y_{ee}|$ & $< |y_{ee}|$ & $< |y_{ee}|$ & $< |y_{ee}|$ & $< |y_{ee}|$ & $< |y_{ee}|$ & $< |y_{ee}|$ & $< |y_{ee}|$ & $< |y_{ee}|$ & $< |\Delta \eta_{ee}|$ & $< |\Delta \eta_{ee}|$ & $< |\Delta \eta_{ee}|$ & $< |\Delta \eta_{ee}|$ & $< |\Delta \eta_{ee}|$ & $< |\Delta \eta_{ee}|$ & $< |\Delta \eta_{ee}|$ & $< |\Delta \eta_{ee}|$ & $< |\Delta \eta_{ee}|$ & $< |\Delta \eta_{ee}|$ & $< |\Delta \eta_{ee}|$ & $< |\Delta \eta_{ee}|$\\
  & $< 130~\GeV$ & $< 150~\GeV$ & $< 0.2$ & $< 0.4$ & $< 0.6$ & $< 0.8$ & $< 1.0$ & $< 1.2$ & $< 1.4$ & $< 1.6$ & $< 1.8$ & $< 2.0$ & $< 2.2$ & $< 2.4$ & $< 0.25$ & $< 0.5$ & $< 0.75$ & $< 1.0$ & $< 1.25$ & $< 1.5$ & $< 1.75$ & $< 2.0$ & $< 2.25$ & $< 2.5$ & $< 2.75$ & $< 3.0$\\\hline
$116~\GeV < m_{ee} < 130~\GeV$ & 1.00 & 0.02 & 0.29 & 0.27 & 0.27 & 0.26 & 0.25 & 0.24 & 0.23 & 0.23 & 0.19 & 0.16 & 0.17 & 0.09 & 0.32 & 0.31 & 0.30 & 0.28 & 0.28 & 0.26 & 0.22 & 0.22 & 0.11 & 0.03 & 0.00 & -0.00\\
$130~\GeV < m_{ee} < 150~\GeV$ & 0.02 & 1.00 & 0.22 & 0.24 & 0.24 & 0.22 & 0.22 & 0.22 & 0.19 & 0.19 & 0.17 & 0.13 & 0.11 & 0.06 & 0.25 & 0.25 & 0.23 & 0.24 & 0.20 & 0.23 & 0.20 & 0.17 & 0.19 & 0.14 & 0.05 & 0.03\\
$0.0 < |y_{ee}| < 0.2$ & 0.29 & 0.22 & 1.00 & 0.00 & 0.01 & 0.00 & -0.01 & 0.01 & -0.01 & 0.01 & -0.00 & -0.02 & 0.02 & -0.00 & 0.11 & 0.12 & 0.13 & 0.14 & 0.12 & 0.13 & 0.12 & 0.12 & 0.08 & 0.04 & 0.01 & 0.01\\
$0.2 < |y_{ee}| < 0.4$ & 0.27 & 0.24 & 0.00 & 1.00 & 0.02 & 0.01 & 0.00 & 0.03 & -0.00 & 0.02 & -0.00 & -0.01 & 0.00 & -0.04 & 0.12 & 0.13 & 0.14 & 0.12 & 0.13 & 0.15 & 0.13 & 0.10 & 0.05 & 0.04 & 0.03 & 0.01\\
$0.4 < |y_{ee}| < 0.6$ & 0.27 & 0.24 & 0.01 & 0.02 & 1.00 & 0.03 & 0.02 & 0.00 & -0.00 & 0.00 & -0.00 & 0.01 & 0.01 & 0.00 & 0.14 & 0.14 & 0.14 & 0.14 & 0.11 & 0.13 & 0.11 & 0.06 & 0.07 & 0.08 & 0.02 & -0.00\\
$0.6 < |y_{ee}| < 0.8$ & 0.26 & 0.22 & 0.00 & 0.01 & 0.03 & 1.00 & -0.00 & -0.01 & 0.01 & 0.01 & 0.01 & -0.02 & 0.01 & -0.00 & 0.12 & 0.13 & 0.13 & 0.16 & 0.11 & 0.07 & 0.08 & 0.10 & 0.10 & 0.06 & 0.03 & 0.02\\
$0.8 < |y_{ee}| < 1.0$ & 0.25 & 0.22 & -0.01 & 0.00 & 0.02 & -0.00 & 1.00 & -0.00 & 0.00 & 0.01 & 0.02 & -0.00 & 0.00 & 0.01 & 0.13 & 0.12 & 0.14 & 0.09 & 0.07 & 0.11 & 0.10 & 0.12 & 0.11 & 0.06 & 0.02 & 0.03\\
$1.0 < |y_{ee}| < 1.2$ & 0.24 & 0.22 & 0.01 & 0.03 & 0.00 & -0.01 & -0.00 & 1.00 & -0.00 & -0.00 & 0.00 & 0.00 & 0.01 & -0.01 & 0.13 & 0.12 & 0.05 & 0.08 & 0.12 & 0.14 & 0.13 & 0.13 & 0.09 & 0.06 & 0.01 & -0.01\\
$1.2 < |y_{ee}| < 1.4$ & 0.23 & 0.19 & -0.01 & -0.00 & -0.00 & 0.01 & 0.00 & -0.00 & 1.00 & 0.01 & -0.01 & 0.00 & 0.01 & 0.01 & 0.07 & 0.07 & 0.09 & 0.13 & 0.12 & 0.13 & 0.12 & 0.11 & 0.10 & 0.04 & -0.02 & 0.01\\
$1.4 < |y_{ee}| < 1.6$ & 0.23 & 0.19 & 0.01 & 0.02 & 0.00 & 0.01 & 0.01 & -0.00 & 0.01 & 1.00 & -0.01 & -0.01 & 0.00 & -0.01 & 0.03 & 0.10 & 0.13 & 0.12 & 0.15 & 0.14 & 0.13 & 0.07 & 0.03 & -0.01 & -0.00 & 0.00\\
$1.6 < |y_{ee}| < 1.8$ & 0.19 & 0.17 & -0.00 & -0.00 & -0.00 & 0.01 & 0.02 & 0.00 & -0.01 & -0.01 & 1.00 & 0.02 & 0.01 & 0.01 & 0.13 & 0.07 & 0.08 & 0.14 & 0.15 & 0.09 & 0.04 & 0.02 & 0.00 & 0.00 & 0.01 & 0.01\\
$1.8 < |y_{ee}| < 2.0$ & 0.16 & 0.13 & -0.02 & -0.01 & 0.01 & -0.02 & -0.00 & 0.00 & 0.00 & -0.01 & 0.02 & 1.00 & -0.02 & 0.00 & 0.14 & 0.14 & 0.13 & 0.06 & 0.06 & 0.02 & -0.01 & 0.01 & 0.02 & -0.02 & -0.01 & -0.01\\
$2.0 < |y_{ee}| < 2.2$ & 0.17 & 0.11 & 0.02 & 0.00 & 0.01 & 0.01 & 0.00 & 0.01 & 0.01 & 0.00 & 0.01 & -0.02 & 1.00 & 0.00 & 0.19 & 0.18 & 0.12 & 0.03 & 0.01 & -0.01 & 0.00 & 0.01 & 0.01 & -0.00 & 0.00 & -0.01\\
$2.2 < |y_{ee}| < 2.4$ & 0.09 & 0.06 & -0.00 & -0.04 & 0.00 & -0.00 & 0.01 & -0.01 & 0.01 & -0.01 & 0.01 & 0.00 & 0.00 & 1.00 & 0.21 & 0.10 & -0.00 & 0.02 & -0.02 & -0.00 & -0.01 & -0.00 & -0.01 & -0.00 & -0.00 & -0.02\\
$0.0 < |\Delta \eta_{ee}| < 0.25$ & 0.32 & 0.25 & 0.11 & 0.12 & 0.14 & 0.12 & 0.13 & 0.13 & 0.07 & 0.03 & 0.13 & 0.14 & 0.19 & 0.21 & 1.00 & 0.00 & 0.00 & 0.00 & -0.02 & 0.02 & 0.01 & 0.02 & 0.01 & -0.00 & 0.00 & -0.01\\
$0.25 < |\Delta \eta_{ee}| < 0.5$ & 0.31 & 0.25 & 0.12 & 0.13 & 0.14 & 0.13 & 0.12 & 0.12 & 0.07 & 0.10 & 0.07 & 0.14 & 0.18 & 0.10 & 0.00 & 1.00 & 0.01 & 0.01 & -0.01 & -0.00 & 0.02 & 0.01 & 0.01 & -0.01 & -0.02 & 0.01\\
$0.5 < |\Delta \eta_{ee}| < 0.75$ & 0.30 & 0.23 & 0.13 & 0.14 & 0.14 & 0.13 & 0.14 & 0.05 & 0.09 & 0.13 & 0.08 & 0.13 & 0.12 & -0.00 & 0.00 & 0.01 & 1.00 & 0.01 & 0.01 & -0.02 & -0.01 & -0.00 & 0.01 & -0.01 & -0.00 & 0.01\\
$0.75 < |\Delta \eta_{ee}| < 1.0$ & 0.28 & 0.24 & 0.14 & 0.12 & 0.14 & 0.16 & 0.09 & 0.08 & 0.13 & 0.12 & 0.14 & 0.06 & 0.03 & 0.02 & 0.00 & 0.01 & 0.01 & 1.00 & 0.01 & 0.01 & -0.02 & 0.01 & 0.01 & 0.01 & -0.01 & 0.02\\
$1.0 < |\Delta \eta_{ee}| < 1.25$ & 0.28 & 0.20 & 0.12 & 0.13 & 0.11 & 0.11 & 0.07 & 0.12 & 0.12 & 0.15 & 0.15 & 0.06 & 0.01 & -0.02 & -0.02 & -0.01 & 0.01 & 0.01 & 1.00 & 0.01 & 0.02 & -0.00 & 0.00 & 0.01 & 0.00 & -0.01\\
$1.25 < |\Delta \eta_{ee}| < 1.5$ & 0.26 & 0.23 & 0.13 & 0.15 & 0.13 & 0.07 & 0.11 & 0.14 & 0.13 & 0.14 & 0.09 & 0.02 & -0.01 & -0.00 & 0.02 & -0.00 & -0.02 & 0.01 & 0.01 & 1.00 & 0.01 & 0.02 & 0.01 & -0.00 & 0.00 & -0.00\\
$1.5 < |\Delta \eta_{ee}| < 1.75$ & 0.22 & 0.20 & 0.12 & 0.13 & 0.11 & 0.08 & 0.10 & 0.13 & 0.12 & 0.13 & 0.04 & -0.01 & 0.00 & -0.01 & 0.01 & 0.02 & -0.01 & -0.02 & 0.02 & 0.01 & 1.00 & 0.00 & -0.02 & -0.01 & -0.02 & 0.00\\
$1.75 < |\Delta \eta_{ee}| < 2.0$ & 0.22 & 0.17 & 0.12 & 0.10 & 0.06 & 0.10 & 0.12 & 0.13 & 0.11 & 0.07 & 0.02 & 0.01 & 0.01 & -0.00 & 0.02 & 0.01 & -0.00 & 0.01 & -0.00 & 0.02 & 0.00 & 1.00 & -0.00 & -0.01 & -0.02 & 0.00\\
$2.0 < |\Delta \eta_{ee}| < 2.25$ & 0.11 & 0.19 & 0.08 & 0.05 & 0.07 & 0.10 & 0.11 & 0.09 & 0.10 & 0.03 & 0.00 & 0.02 & 0.01 & -0.01 & 0.01 & 0.01 & 0.01 & 0.01 & 0.00 & 0.01 & -0.02 & -0.00 & 1.00 & 0.01 & -0.00 & 0.00\\
$2.25 < |\Delta \eta_{ee}| < 2.5$ & 0.03 & 0.14 & 0.04 & 0.04 & 0.08 & 0.06 & 0.06 & 0.06 & 0.04 & -0.01 & 0.00 & -0.02 & -0.00 & -0.00 & -0.00 & -0.01 & -0.01 & 0.01 & 0.01 & -0.00 & -0.01 & -0.01 & 0.01 & 1.00 & -0.01 & -0.03\\
$2.5 < |\Delta \eta_{ee}| < 2.75$ & 0.00 & 0.05 & 0.01 & 0.03 & 0.02 & 0.03 & 0.02 & 0.01 & -0.02 & -0.00 & 0.01 & -0.01 & 0.00 & -0.00 & 0.00 & -0.02 & -0.00 & -0.01 & 0.00 & 0.00 & -0.02 & -0.02 & -0.00 & -0.01 & 1.00 & -0.01\\
$2.75 < |\Delta \eta_{ee}| < 3.0$ & -0.00 & 0.03 & 0.01 & 0.01 & -0.00 & 0.02 & 0.03 & -0.01 & 0.01 & 0.00 & 0.01 & -0.01 & -0.01 & -0.02 & -0.01 & 0.01 & 0.01 & 0.02 & -0.01 & -0.00 & 0.00 & 0.00 & 0.00 & -0.03 & -0.01 & 1.00\\
\end{tabular} }
\caption{Statistical correlation between the measurement bins in mass, rapidity and $\Delta \eta$ in the electron channel for 116~GeV < \mll\ < 150~GeV.}
\label{table:elec_corr_116to150}
\end{center}
\end{sidewaystable}


==> Shared/tables/electrons/Correlation_elec_150to200.tex <==
\begin{sidewaystable}[!htb]
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|cccccccccccccccccccccccccc|}
  & $150~\GeV$ & $175~\GeV$ & $0.0$ & $0.2$ & $0.4$ & $0.6$ & $0.8$ & $1.0$ & $1.2$ & $1.4$ & $1.6$ & $1.8$ & $2.0$ & $2.2$ & $0.0$ & $0.25$ & $0.5$ & $0.75$ & $1.0$ & $1.25$ & $1.5$ & $1.75$ & $2.0$ & $2.25$ & $2.5$ & $2.75$\\
 Bin & $< m_{ee}$ & $< m_{ee}$ & $< |y_{ee}|$ & $< |y_{ee}|$ & $< |y_{ee}|$ & $< |y_{ee}|$ & $< |y_{ee}|$ & $< |y_{ee}|$ & $< |y_{ee}|$ & $< |y_{ee}|$ & $< |y_{ee}|$ & $< |y_{ee}|$ & $< |y_{ee}|$ & $< |y_{ee}|$ & $< |\Delta \eta_{ee}|$ & $< |\Delta \eta_{ee}|$ & $< |\Delta \eta_{ee}|$ & $< |\Delta \eta_{ee}|$ & $< |\Delta \eta_{ee}|$ & $< |\Delta \eta_{ee}|$ & $< |\Delta \eta_{ee}|$ & $< |\Delta \eta_{ee}|$ & $< |\Delta \eta_{ee}|$ & $< |\Delta \eta_{ee}|$ & $< |\Delta \eta_{ee}|$ & $< |\Delta \eta_{ee}|$\\
  & $< 175~\GeV$ & $< 200~\GeV$ & $< 0.2$ & $< 0.4$ & $< 0.6$ & $< 0.8$ & $< 1.0$ & $< 1.2$ & $< 1.4$ & $< 1.6$ & $< 1.8$ & $< 2.0$ & $< 2.2$ & $< 2.4$ & $< 0.25$ & $< 0.5$ & $< 0.75$ & $< 1.0$ & $< 1.25$ & $< 1.5$ & $< 1.75$ & $< 2.0$ & $< 2.25$ & $< 2.5$ & $< 2.75$ & $< 3.0$\\\hline
$150~\GeV < m_{ee} < 175~\GeV$ & 1.00 & 0.01 & 0.28 & 0.30 & 0.27 & 0.27 & 0.27 & 0.25 & 0.23 & 0.22 & 0.19 & 0.18 & 0.16 & 0.09 & 0.30 & 0.30 & 0.29 & 0.27 & 0.26 & 0.24 & 0.24 & 0.21 & 0.19 & 0.16 & 0.14 & 0.05\\
$175~\GeV < m_{ee} < 200~\GeV$ & 0.01 & 1.00 & 0.22 & 0.22 & 0.22 & 0.21 & 0.20 & 0.18 & 0.18 & 0.15 & 0.15 & 0.11 & 0.10 & 0.07 & 0.21 & 0.21 & 0.20 & 0.18 & 0.20 & 0.18 & 0.19 & 0.16 & 0.12 & 0.13 & 0.13 & 0.12\\
$0.0 < |y_{ee}| < 0.2$ & 0.28 & 0.22 & 1.00 & 0.01 & 0.01 & -0.01 & 0.02 & 0.00 & -0.01 & 0.01 & -0.01 & -0.00 & -0.00 & 0.01 & 0.09 & 0.14 & 0.10 & 0.11 & 0.13 & 0.13 & 0.12 & 0.12 & 0.09 & 0.07 & 0.06 & 0.05\\
$0.2 < |y_{ee}| < 0.4$ & 0.30 & 0.22 & 0.01 & 1.00 & 0.00 & 0.01 & -0.00 & -0.00 & 0.02 & 0.01 & -0.00 & 0.01 & 0.01 & -0.00 & 0.13 & 0.11 & 0.13 & 0.10 & 0.13 & 0.12 & 0.12 & 0.11 & 0.08 & 0.08 & 0.08 & 0.07\\
$0.4 < |y_{ee}| < 0.6$ & 0.27 & 0.22 & 0.01 & 0.00 & 1.00 & -0.01 & -0.00 & -0.00 & -0.01 & 0.00 & 0.01 & 0.00 & 0.00 & -0.01 & 0.11 & 0.11 & 0.13 & 0.12 & 0.11 & 0.12 & 0.10 & 0.08 & 0.07 & 0.09 & 0.08 & 0.06\\
$0.6 < |y_{ee}| < 0.8$ & 0.27 & 0.21 & -0.01 & 0.01 & -0.01 & 1.00 & -0.01 & 0.00 & 0.01 & -0.00 & -0.01 & 0.00 & 0.01 & -0.00 & 0.10 & 0.12 & 0.12 & 0.12 & 0.09 & 0.07 & 0.08 & 0.09 & 0.10 & 0.10 & 0.11 & 0.06\\
$0.8 < |y_{ee}| < 1.0$ & 0.27 & 0.20 & 0.02 & -0.00 & -0.00 & -0.01 & 1.00 & -0.01 & -0.02 & -0.01 & 0.02 & 0.00 & 0.01 & 0.00 & 0.12 & 0.13 & 0.09 & 0.10 & 0.05 & 0.08 & 0.09 & 0.11 & 0.10 & 0.10 & 0.11 & 0.05\\
$1.0 < |y_{ee}| < 1.2$ & 0.25 & 0.18 & 0.00 & -0.00 & -0.00 & 0.00 & -0.01 & 1.00 & -0.01 & 0.01 & 0.00 & 0.00 & -0.01 & 0.01 & 0.11 & 0.09 & 0.05 & 0.08 & 0.11 & 0.10 & 0.11 & 0.12 & 0.11 & 0.10 & 0.06 & 0.03\\
$1.2 < |y_{ee}| < 1.4$ & 0.23 & 0.18 & -0.01 & 0.02 & -0.01 & 0.01 & -0.02 & -0.01 & 1.00 & 0.00 & -0.01 & -0.00 & -0.00 & -0.02 & 0.04 & 0.06 & 0.11 & 0.13 & 0.12 & 0.10 & 0.12 & 0.09 & 0.09 & 0.07 & 0.04 & 0.01\\
$1.4 < |y_{ee}| < 1.6$ & 0.22 & 0.15 & 0.01 & 0.01 & 0.00 & -0.00 & -0.01 & 0.01 & 0.00 & 1.00 & 0.00 & -0.02 & 0.02 & -0.01 & 0.01 & 0.10 & 0.12 & 0.12 & 0.12 & 0.11 & 0.14 & 0.07 & 0.04 & 0.01 & -0.02 & 0.02\\
$1.6 < |y_{ee}| < 1.8$ & 0.19 & 0.15 & -0.01 & -0.00 & 0.01 & -0.01 & 0.02 & 0.00 & -0.01 & 0.00 & 1.00 & 0.01 & 0.02 & 0.01 & 0.14 & 0.07 & 0.09 & 0.12 & 0.13 & 0.09 & 0.04 & 0.03 & 0.01 & 0.00 & 0.00 & -0.01\\
$1.8 < |y_{ee}| < 2.0$ & 0.18 & 0.11 & -0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & -0.00 & -0.02 & 0.01 & 1.00 & -0.00 & 0.01 & 0.15 & 0.15 & 0.12 & 0.03 & 0.08 & 0.01 & 0.02 & -0.00 & -0.02 & 0.01 & 0.02 & 0.00\\
$2.0 < |y_{ee}| < 2.2$ & 0.16 & 0.10 & -0.00 & 0.01 & 0.00 & 0.01 & 0.01 & -0.01 & -0.00 & 0.02 & 0.02 & -0.00 & 1.00 & -0.01 & 0.16 & 0.15 & 0.12 & 0.03 & -0.00 & 0.01 & 0.03 & -0.01 & 0.02 & -0.00 & 0.03 & -0.00\\
$2.2 < |y_{ee}| < 2.4$ & 0.09 & 0.07 & 0.01 & -0.00 & -0.01 & -0.00 & 0.00 & 0.01 & -0.02 & -0.01 & 0.01 & 0.01 & -0.01 & 1.00 & 0.20 & 0.08 & 0.01 & -0.01 & 0.01 & 0.00 & 0.01 & -0.01 & 0.01 & 0.01 & -0.00 & -0.00\\
$0.0 < |\Delta \eta_{ee}| < 0.25$ & 0.30 & 0.21 & 0.09 & 0.13 & 0.11 & 0.10 & 0.12 & 0.11 & 0.04 & 0.01 & 0.14 & 0.15 & 0.16 & 0.20 & 1.00 & -0.01 & 0.00 & -0.01 & -0.01 & -0.02 & 0.01 & -0.01 & -0.01 & 0.00 & -0.00 & -0.00\\
$0.25 < |\Delta \eta_{ee}| < 0.5$ & 0.30 & 0.21 & 0.14 & 0.11 & 0.11 & 0.12 & 0.13 & 0.09 & 0.06 & 0.10 & 0.07 & 0.15 & 0.15 & 0.08 & -0.01 & 1.00 & -0.01 & 0.00 & 0.00 & -0.01 & 0.01 & 0.02 & 0.00 & -0.00 & 0.02 & 0.01\\
$0.5 < |\Delta \eta_{ee}| < 0.75$ & 0.29 & 0.20 & 0.10 & 0.13 & 0.13 & 0.12 & 0.09 & 0.05 & 0.11 & 0.12 & 0.09 & 0.12 & 0.12 & 0.01 & 0.00 & -0.01 & 1.00 & -0.02 & 0.01 & -0.01 & 0.01 & -0.00 & 0.01 & 0.02 & 0.00 & -0.00\\
$0.75 < |\Delta \eta_{ee}| < 1.0$ & 0.27 & 0.18 & 0.11 & 0.10 & 0.12 & 0.12 & 0.10 & 0.08 & 0.13 & 0.12 & 0.12 & 0.03 & 0.03 & -0.01 & -0.01 & 0.00 & -0.02 & 1.00 & -0.01 & -0.00 & 0.01 & 0.00 & -0.02 & 0.00 & 0.00 & -0.02\\
$1.0 < |\Delta \eta_{ee}| < 1.25$ & 0.26 & 0.20 & 0.13 & 0.13 & 0.11 & 0.09 & 0.05 & 0.11 & 0.12 & 0.12 & 0.13 & 0.08 & -0.00 & 0.01 & -0.01 & 0.00 & 0.01 & -0.01 & 1.00 & 0.01 & 0.01 & -0.01 & 0.01 & -0.00 & -0.00 & -0.00\\
$1.25 < |\Delta \eta_{ee}| < 1.5$ & 0.24 & 0.18 & 0.13 & 0.12 & 0.12 & 0.07 & 0.08 & 0.10 & 0.10 & 0.11 & 0.09 & 0.01 & 0.01 & 0.00 & -0.02 & -0.01 & -0.01 & -0.00 & 0.01 & 1.00 & -0.01 & 0.01 & -0.00 & 0.00 & -0.00 & 0.02\\
$1.5 < |\Delta \eta_{ee}| < 1.75$ & 0.24 & 0.19 & 0.12 & 0.12 & 0.10 & 0.08 & 0.09 & 0.11 & 0.12 & 0.14 & 0.04 & 0.02 & 0.03 & 0.01 & 0.01 & 0.01 & 0.01 & 0.01 & 0.01 & -0.01 & 1.00 & 0.00 & -0.01 & -0.00 & 0.01 & 0.01\\
$1.75 < |\Delta \eta_{ee}| < 2.0$ & 0.21 & 0.16 & 0.12 & 0.11 & 0.08 & 0.09 & 0.11 & 0.12 & 0.09 & 0.07 & 0.03 & -0.00 & -0.01 & -0.01 & -0.01 & 0.02 & -0.00 & 0.00 & -0.01 & 0.01 & 0.00 & 1.00 & 0.01 & -0.01 & 0.02 & -0.01\\
$2.0 < |\Delta \eta_{ee}| < 2.25$ & 0.19 & 0.12 & 0.09 & 0.08 & 0.07 & 0.10 & 0.10 & 0.11 & 0.09 & 0.04 & 0.01 & -0.02 & 0.02 & 0.01 & -0.01 & 0.00 & 0.01 & -0.02 & 0.01 & -0.00 & -0.01 & 0.01 & 1.00 & 0.01 & -0.00 & -0.02\\
$2.25 < |\Delta \eta_{ee}| < 2.5$ & 0.16 & 0.13 & 0.07 & 0.08 & 0.09 & 0.10 & 0.10 & 0.10 & 0.07 & 0.01 & 0.00 & 0.01 & -0.00 & 0.01 & 0.00 & -0.00 & 0.02 & 0.00 & -0.00 & 0.00 & -0.00 & -0.01 & 0.01 & 1.00 & 0.00 & -0.01\\
$2.5 < |\Delta \eta_{ee}| < 2.75$ & 0.14 & 0.13 & 0.06 & 0.08 & 0.08 & 0.11 & 0.11 & 0.06 & 0.04 & -0.02 & 0.00 & 0.02 & 0.03 & -0.00 & -0.00 & 0.02 & 0.00 & 0.00 & -0.00 & -0.00 & 0.01 & 0.02 & -0.00 & 0.00 & 1.00 & 0.01\\
$2.75 < |\Delta \eta_{ee}| < 3.0$ & 0.05 & 0.12 & 0.05 & 0.07 & 0.06 & 0.06 & 0.05 & 0.03 & 0.01 & 0.02 & -0.01 & 0.00 & -0.00 & -0.00 & -0.00 & 0.01 & -0.00 & -0.02 & -0.00 & 0.02 & 0.01 & -0.01 & -0.02 & -0.01 & 0.01 & 1.00\\
\end{tabular} }
\caption{Statistical correlation between the measurement bins in mass, rapidity and $\Delta \eta$ in the electron channel for 150~GeV < \mll\ < 200~GeV.}
\label{table:elec_corr_150to200}
\end{center}
\end{sidewaystable}


==> Shared/tables/electrons/Correlation_elec_200to300.tex <==
\begin{sidewaystable}[!htb]
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|ccccccccccccccccccccccccccc|}
  & $200~\GeV$ & $230~\GeV$ & $260~\GeV$ & $0.0$ & $0.2$ & $0.4$ & $0.6$ & $0.8$ & $1.0$ & $1.2$ & $1.4$ & $1.6$ & $1.8$ & $2.0$ & $2.2$ & $0.0$ & $0.25$ & $0.5$ & $0.75$ & $1.0$ & $1.25$ & $1.5$ & $1.75$ & $2.0$ & $2.25$ & $2.5$ & $2.75$\\
 Bin & $< m_{ee}$ & $< m_{ee}$ & $< m_{ee}$ & $< |y_{ee}|$ & $< |y_{ee}|$ & $< |y_{ee}|$ & $< |y_{ee}|$ & $< |y_{ee}|$ & $< |y_{ee}|$ & $< |y_{ee}|$ & $< |y_{ee}|$ & $< |y_{ee}|$ & $< |y_{ee}|$ & $< |y_{ee}|$ & $< |y_{ee}|$ & $< |\Delta \eta_{ee}|$ & $< |\Delta \eta_{ee}|$ & $< |\Delta \eta_{ee}|$ & $< |\Delta \eta_{ee}|$ & $< |\Delta \eta_{ee}|$ & $< |\Delta \eta_{ee}|$ & $< |\Delta \eta_{ee}|$ & $< |\Delta \eta_{ee}|$ & $< |\Delta \eta_{ee}|$ & $< |\Delta \eta_{ee}|$ & $< |\Delta \eta_{ee}|$ & $< |\Delta \eta_{ee}|$\\
  & $< 230~\GeV$ & $< 260~\GeV$ & $< 300~\GeV$ & $< 0.2$ & $< 0.4$ & $< 0.6$ & $< 0.8$ & $< 1.0$ & $< 1.2$ & $< 1.4$ & $< 1.6$ & $< 1.8$ & $< 2.0$ & $< 2.2$ & $< 2.4$ & $< 0.25$ & $< 0.5$ & $< 0.75$ & $< 1.0$ & $< 1.25$ & $< 1.5$ & $< 1.75$ & $< 2.0$ & $< 2.25$ & $< 2.5$ & $< 2.75$ & $< 3.0$\\\hline
$200~\GeV < m_{ee} < 230~\GeV$ & 1.00 & 0.01 & 0.00 & 0.26 & 0.25 & 0.26 & 0.27 & 0.24 & 0.22 & 0.20 & 0.19 & 0.16 & 0.14 & 0.11 & 0.07 & 0.26 & 0.25 & 0.24 & 0.24 & 0.23 & 0.22 & 0.20 & 0.18 & 0.16 & 0.14 & 0.13 & 0.12\\
$230~\GeV < m_{ee} < 260~\GeV$ & 0.01 & 1.00 & 0.02 & 0.18 & 0.21 & 0.21 & 0.18 & 0.18 & 0.18 & 0.17 & 0.13 & 0.12 & 0.10 & 0.09 & 0.06 & 0.18 & 0.19 & 0.17 & 0.19 & 0.16 & 0.15 & 0.15 & 0.13 & 0.14 & 0.12 & 0.11 & 0.11\\
$260~\GeV < m_{ee} < 300~\GeV$ & 0.00 & 0.02 & 1.00 & 0.17 & 0.16 & 0.19 & 0.19 & 0.17 & 0.13 & 0.14 & 0.13 & 0.11 & 0.07 & 0.08 & 0.06 & 0.16 & 0.16 & 0.15 & 0.15 & 0.17 & 0.14 & 0.13 & 0.11 & 0.13 & 0.11 & 0.10 & 0.10\\
$0.0 < |y_{ee}| < 0.2$ & 0.26 & 0.18 & 0.17 & 1.00 & 0.01 & 0.00 & -0.01 & -0.01 & -0.01 & 0.01 & 0.01 & -0.00 & 0.01 & -0.01 & 0.02 & 0.12 & 0.10 & 0.11 & 0.13 & 0.12 & 0.10 & 0.12 & 0.09 & 0.09 & 0.08 & 0.07 & 0.08\\
$0.2 < |y_{ee}| < 0.4$ & 0.25 & 0.21 & 0.16 & 0.01 & 1.00 & 0.01 & -0.01 & 0.00 & 0.01 & 0.01 & 0.00 & -0.01 & -0.01 & 0.01 & 0.00 & 0.10 & 0.11 & 0.09 & 0.12 & 0.13 & 0.12 & 0.12 & 0.07 & 0.12 & 0.06 & 0.10 & 0.07\\
$0.4 < |y_{ee}| < 0.6$ & 0.26 & 0.21 & 0.19 & 0.00 & 0.01 & 1.00 & 0.02 & 0.01 & -0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.13 & 0.13 & 0.12 & 0.13 & 0.11 & 0.12 & 0.09 & 0.05 & 0.07 & 0.10 & 0.08 & 0.11\\
$0.6 < |y_{ee}| < 0.8$ & 0.27 & 0.18 & 0.19 & -0.01 & -0.01 & 0.02 & 1.00 & 0.00 & 0.00 & 0.01 & 0.01 & 0.02 & 0.01 & 0.02 & 0.02 & 0.12 & 0.14 & 0.12 & 0.13 & 0.11 & 0.06 & 0.06 & 0.09 & 0.12 & 0.09 & 0.09 & 0.12\\
$0.8 < |y_{ee}| < 1.0$ & 0.24 & 0.18 & 0.17 & -0.01 & 0.00 & 0.01 & 0.00 & 1.00 & -0.00 & 0.01 & -0.01 & 0.01 & 0.00 & 0.00 & -0.01 & 0.10 & 0.11 & 0.10 & 0.09 & 0.06 & 0.08 & 0.10 & 0.13 & 0.11 & 0.11 & 0.10 & 0.09\\
$1.0 < |y_{ee}| < 1.2$ & 0.22 & 0.18 & 0.13 & -0.01 & 0.01 & -0.00 & 0.00 & -0.00 & 1.00 & 0.00 & -0.01 & 0.00 & -0.01 & 0.00 & -0.01 & 0.10 & 0.10 & 0.05 & 0.04 & 0.11 & 0.12 & 0.12 & 0.10 & 0.13 & 0.09 & 0.09 & 0.03\\
$1.2 < |y_{ee}| < 1.4$ & 0.20 & 0.17 & 0.14 & 0.01 & 0.01 & 0.00 & 0.01 & 0.01 & 0.00 & 1.00 & 0.01 & -0.00 & -0.00 & 0.00 & 0.01 & 0.07 & 0.06 & 0.11 & 0.10 & 0.13 & 0.13 & 0.10 & 0.12 & 0.08 & 0.06 & 0.03 & 0.03\\
$1.4 < |y_{ee}| < 1.6$ & 0.19 & 0.13 & 0.13 & 0.01 & 0.00 & 0.01 & 0.01 & -0.01 & -0.01 & 0.01 & 1.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.03 & 0.09 & 0.11 & 0.13 & 0.13 & 0.11 & 0.13 & 0.08 & 0.02 & 0.03 & 0.01 & 0.01\\
$1.6 < |y_{ee}| < 1.8$ & 0.16 & 0.12 & 0.11 & -0.00 & -0.01 & 0.00 & 0.02 & 0.01 & 0.00 & -0.00 & 0.01 & 1.00 & -0.00 & -0.01 & 0.00 & 0.12 & 0.06 & 0.08 & 0.15 & 0.13 & 0.10 & 0.06 & 0.02 & 0.01 & -0.01 & -0.01 & 0.00\\
$1.8 < |y_{ee}| < 2.0$ & 0.14 & 0.10 & 0.07 & 0.01 & -0.01 & 0.00 & 0.01 & 0.00 & -0.01 & -0.00 & 0.00 & -0.00 & 1.00 & -0.00 & 0.02 & 0.16 & 0.16 & 0.12 & 0.06 & 0.06 & 0.01 & -0.00 & 0.00 & 0.01 & -0.01 & 0.02 & -0.02\\
$2.0 < |y_{ee}| < 2.2$ & 0.11 & 0.09 & 0.08 & -0.01 & 0.01 & 0.00 & 0.02 & 0.00 & 0.00 & 0.00 & 0.00 & -0.01 & -0.00 & 1.00 & -0.00 & 0.15 & 0.17 & 0.11 & 0.04 & -0.00 & 0.00 & -0.01 & 0.01 & -0.01 & 0.01 & 0.01 & -0.00\\
$2.2 < |y_{ee}| < 2.4$ & 0.07 & 0.06 & 0.06 & 0.02 & 0.00 & 0.00 & 0.02 & -0.01 & -0.01 & 0.01 & 0.00 & 0.00 & 0.02 & -0.00 & 1.00 & 0.18 & 0.10 & 0.03 & 0.01 & 0.00 & -0.00 & 0.01 & -0.00 & -0.01 & 0.01 & -0.00 & 0.01\\
$0.0 < |\Delta \eta_{ee}| < 0.25$ & 0.26 & 0.18 & 0.16 & 0.12 & 0.10 & 0.13 & 0.12 & 0.10 & 0.10 & 0.07 & 0.03 & 0.12 & 0.16 & 0.15 & 0.18 & 1.00 & 0.01 & 0.01 & 0.01 & 0.01 & 0.01 & -0.00 & 0.01 & 0.01 & -0.01 & -0.01 & -0.01\\
$0.25 < |\Delta \eta_{ee}| < 0.5$ & 0.25 & 0.19 & 0.16 & 0.10 & 0.11 & 0.13 & 0.14 & 0.11 & 0.10 & 0.06 & 0.09 & 0.06 & 0.16 & 0.17 & 0.10 & 0.01 & 1.00 & 0.01 & 0.02 & -0.00 & 0.02 & 0.00 & -0.00 & -0.00 & 0.00 & -0.02 & 0.01\\
$0.5 < |\Delta \eta_{ee}| < 0.75$ & 0.24 & 0.17 & 0.15 & 0.11 & 0.09 & 0.12 & 0.12 & 0.10 & 0.05 & 0.11 & 0.11 & 0.08 & 0.12 & 0.11 & 0.03 & 0.01 & 0.01 & 1.00 & 0.00 & -0.01 & -0.00 & -0.00 & -0.00 & 0.01 & 0.00 & -0.00 & -0.01\\
$0.75 < |\Delta \eta_{ee}| < 1.0$ & 0.24 & 0.19 & 0.15 & 0.13 & 0.12 & 0.13 & 0.13 & 0.09 & 0.04 & 0.10 & 0.13 & 0.15 & 0.06 & 0.04 & 0.01 & 0.01 & 0.02 & 0.00 & 1.00 & -0.00 & -0.01 & 0.01 & 0.00 & 0.01 & -0.02 & 0.02 & 0.01\\
$1.0 < |\Delta \eta_{ee}| < 1.25$ & 0.23 & 0.16 & 0.17 & 0.12 & 0.13 & 0.11 & 0.11 & 0.06 & 0.11 & 0.13 & 0.13 & 0.13 & 0.06 & -0.00 & 0.00 & 0.01 & -0.00 & -0.01 & -0.00 & 1.00 & 0.00 & 0.01 & 0.01 & 0.01 & 0.01 & 0.00 & -0.00\\
$1.25 < |\Delta \eta_{ee}| < 1.5$ & 0.22 & 0.15 & 0.14 & 0.10 & 0.12 & 0.12 & 0.06 & 0.08 & 0.12 & 0.13 & 0.11 & 0.10 & 0.01 & 0.00 & -0.00 & 0.01 & 0.02 & -0.00 & -0.01 & 0.00 & 1.00 & -0.00 & -0.03 & -0.00 & -0.00 & 0.01 & 0.00\\
$1.5 < |\Delta \eta_{ee}| < 1.75$ & 0.20 & 0.15 & 0.13 & 0.12 & 0.12 & 0.09 & 0.06 & 0.10 & 0.12 & 0.10 & 0.13 & 0.06 & -0.00 & -0.01 & 0.01 & -0.00 & 0.00 & -0.00 & 0.01 & 0.01 & -0.00 & 1.00 & -0.01 & -0.01 & -0.01 & 0.02 & 0.01\\
$1.75 < |\Delta \eta_{ee}| < 2.0$ & 0.18 & 0.13 & 0.11 & 0.09 & 0.07 & 0.05 & 0.09 & 0.13 & 0.10 & 0.12 & 0.08 & 0.02 & 0.00 & 0.01 & -0.00 & 0.01 & -0.00 & -0.00 & 0.00 & 0.01 & -0.03 & -0.01 & 1.00 & -0.00 & -0.00 & 0.00 & 0.01\\
$2.0 < |\Delta \eta_{ee}| < 2.25$ & 0.16 & 0.14 & 0.13 & 0.09 & 0.12 & 0.07 & 0.12 & 0.11 & 0.13 & 0.08 & 0.02 & 0.01 & 0.01 & -0.01 & -0.01 & 0.01 & -0.00 & 0.01 & 0.01 & 0.01 & -0.00 & -0.01 & -0.00 & 1.00 & 0.01 & -0.01 & -0.02\\
$2.25 < |\Delta \eta_{ee}| < 2.5$ & 0.14 & 0.12 & 0.11 & 0.08 & 0.06 & 0.10 & 0.09 & 0.11 & 0.09 & 0.06 & 0.03 & -0.01 & -0.01 & 0.01 & 0.01 & -0.01 & 0.00 & 0.00 & -0.02 & 0.01 & -0.00 & -0.01 & -0.00 & 0.01 & 1.00 & -0.01 & 0.00\\
$2.5 < |\Delta \eta_{ee}| < 2.75$ & 0.13 & 0.11 & 0.10 & 0.07 & 0.10 & 0.08 & 0.09 & 0.10 & 0.09 & 0.03 & 0.01 & -0.01 & 0.02 & 0.01 & -0.00 & -0.01 & -0.02 & -0.00 & 0.02 & 0.00 & 0.01 & 0.02 & 0.00 & -0.01 & -0.01 & 1.00 & -0.01\\
$2.75 < |\Delta \eta_{ee}| < 3.0$ & 0.12 & 0.11 & 0.10 & 0.08 & 0.07 & 0.11 & 0.12 & 0.09 & 0.03 & 0.03 & 0.01 & 0.00 & -0.02 & -0.00 & 0.01 & -0.01 & 0.01 & -0.01 & 0.01 & -0.00 & 0.00 & 0.01 & 0.01 & -0.02 & 0.00 & -0.01 & 1.00\\
\end{tabular} }
\caption{Statistical correlation between the measurement bins in mass, rapidity and $\Delta \eta$ in the electron channel for 200~GeV < \mll\ < 300~GeV.}
\label{table:elec_corr_200to300}
\end{center}
\end{sidewaystable}


==> Shared/tables/electrons/Correlation_elec_300to500.tex <==
\begin{sidewaystable}[!htb]
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|cccccccccccccc|}
  & $300~\GeV$ & $380~\GeV$ & $0.0$ & $0.4$ & $0.8$ & $1.2$ & $1.6$ & $2.0$ & $0.0$ & $0.5$ & $1.0$ & $1.5$ & $2.0$ & $2.5$\\
 Bin & $< m_{ee}$ & $< m_{ee}$ & $< |y_{ee}|$ & $< |y_{ee}|$ & $< |y_{ee}|$ & $< |y_{ee}|$ & $< |y_{ee}|$ & $< |y_{ee}|$ & $< |\Delta \eta_{ee}|$ & $< |\Delta \eta_{ee}|$ & $< |\Delta \eta_{ee}|$ & $< |\Delta \eta_{ee}|$ & $< |\Delta \eta_{ee}|$ & $< |\Delta \eta_{ee}|$\\
  & $< 380~\GeV$ & $< 500~\GeV$ & $< 0.4$ & $< 0.8$ & $< 1.2$ & $< 1.6$ & $< 2.0$ & $< 2.4$ & $< 0.5$ & $< 1.0$ & $< 1.5$ & $< 2.0$ & $< 2.5$ & $< 3.0$\\\hline
$300~\GeV < m_{ee} < 380~\GeV$ & 1.00 & 0.01 & 0.43 & 0.41 & 0.40 & 0.31 & 0.24 & 0.14 & 0.36 & 0.36 & 0.36 & 0.34 & 0.29 & 0.23\\
$380~\GeV < m_{ee} < 500~\GeV$ & 0.01 & 1.00 & 0.32 & 0.32 & 0.27 & 0.19 & 0.12 & 0.06 & 0.28 & 0.24 & 0.27 & 0.21 & 0.17 & 0.19\\
$0.0 < |y_{ee}| < 0.4$ & 0.43 & 0.32 & 1.00 & 0.00 & 0.01 & -0.00 & 0.00 & -0.00 & 0.22 & 0.19 & 0.24 & 0.22 & 0.20 & 0.17\\
$0.4 < |y_{ee}| < 0.8$ & 0.41 & 0.32 & 0.00 & 1.00 & 0.01 & -0.01 & 0.01 & 0.01 & 0.23 & 0.21 & 0.20 & 0.17 & 0.18 & 0.19\\
$0.8 < |y_{ee}| < 1.2$ & 0.40 & 0.27 & 0.01 & 0.01 & 1.00 & 0.00 & 0.01 & -0.01 & 0.20 & 0.14 & 0.18 & 0.24 & 0.22 & 0.20\\
$1.2 < |y_{ee}| < 1.6$ & 0.31 & 0.19 & -0.00 & -0.01 & 0.00 & 1.00 & -0.01 & 0.00 & 0.10 & 0.24 & 0.24 & 0.20 & 0.11 & 0.02\\
$1.6 < |y_{ee}| < 2.0$ & 0.24 & 0.12 & 0.00 & 0.01 & 0.01 & -0.01 & 1.00 & 0.02 & 0.22 & 0.20 & 0.16 & 0.03 & -0.02 & 0.02\\
$2.0 < |y_{ee}| < 2.4$ & 0.14 & 0.06 & -0.00 & 0.01 & -0.01 & 0.00 & 0.02 & 1.00 & 0.23 & 0.11 & 0.00 & -0.00 & -0.00 & 0.01\\
$0.0 < |\Delta \eta_{ee}| < 0.5$ & 0.36 & 0.28 & 0.22 & 0.23 & 0.20 & 0.10 & 0.22 & 0.23 & 1.00 & 0.01 & -0.00 & -0.01 & 0.01 & 0.01\\
$0.5 < |\Delta \eta_{ee}| < 1.0$ & 0.36 & 0.24 & 0.19 & 0.21 & 0.14 & 0.24 & 0.20 & 0.11 & 0.01 & 1.00 & 0.01 & -0.00 & 0.00 & 0.01\\
$1.0 < |\Delta \eta_{ee}| < 1.5$ & 0.36 & 0.27 & 0.24 & 0.20 & 0.18 & 0.24 & 0.16 & 0.00 & -0.00 & 0.01 & 1.00 & -0.00 & -0.02 & 0.02\\
$1.5 < |\Delta \eta_{ee}| < 2.0$ & 0.34 & 0.21 & 0.22 & 0.17 & 0.24 & 0.20 & 0.03 & -0.00 & -0.01 & -0.00 & -0.00 & 1.00 & 0.02 & 0.01\\
$2.0 < |\Delta \eta_{ee}| < 2.5$ & 0.29 & 0.17 & 0.20 & 0.18 & 0.22 & 0.11 & -0.02 & -0.00 & 0.01 & 0.00 & -0.02 & 0.02 & 1.00 & -0.00\\
$2.5 < |\Delta \eta_{ee}| < 3.0$ & 0.23 & 0.19 & 0.17 & 0.19 & 0.20 & 0.02 & 0.02 & 0.01 & 0.01 & 0.01 & 0.02 & 0.01 & -0.00 & 1.00\\
\end{tabular} }
\caption{Statistical correlation between the measurement bins in mass, rapidity and $\Delta \eta$ in the electron channel for 300~GeV < \mll\ < 500~GeV.}
\label{table:elec_corr_300to500}
\end{center}
\end{sidewaystable}


==> Shared/tables/electrons/Correlation_elec_500to1500.tex <==
\begin{sidewaystable}[!htb]
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|ccccccccccccccc|}
  & $500~\GeV$ & $700~\GeV$ & $1000~\GeV$ & $0.0$ & $0.4$ & $0.8$ & $1.2$ & $1.6$ & $2.0$ & $0.0$ & $0.5$ & $1.0$ & $1.5$ & $2.0$ & $2.5$\\
 Bin & $< m_{ee}$ & $< m_{ee}$ & $< m_{ee}$ & $< |y_{ee}|$ & $< |y_{ee}|$ & $< |y_{ee}|$ & $< |y_{ee}|$ & $< |y_{ee}|$ & $< |y_{ee}|$ & $< |\Delta \eta_{ee}|$ & $< |\Delta \eta_{ee}|$ & $< |\Delta \eta_{ee}|$ & $< |\Delta \eta_{ee}|$ & $< |\Delta \eta_{ee}|$ & $< |\Delta \eta_{ee}|$\\
  & $< 700~\GeV$ & $< 1000~\GeV$ & $< 1500~\GeV$ & $< 0.4$ & $< 0.8$ & $< 1.2$ & $< 1.6$ & $< 2.0$ & $< 2.4$ & $< 0.5$ & $< 1.0$ & $< 1.5$ & $< 2.0$ & $< 2.5$ & $< 3.0$\\\hline
$500~\GeV < m_{ee} < 700~\GeV$ & 1.00 & 0.00 & -0.01 & 0.49 & 0.45 & 0.38 & 0.37 & 0.19 & 0.08 & 0.34 & 0.38 & 0.44 & 0.39 & 0.26 & 0.24\\
$700~\GeV < m_{ee} < 1000~\GeV$ & 0.00 & 1.00 & 0.00 & 0.24 & 0.30 & 0.24 & 0.10 & 0.01 & 0.00 & 0.22 & 0.22 & 0.14 & 0.17 & 0.15 & 0.12\\
$1000~\GeV < m_{ee} < 1500~\GeV$ & -0.01 & 0.00 & 1.00 & 0.14 & 0.13 & 0.06 & 0.04 & -0.01 & -0.00 & 0.15 & 0.11 & 0.06 & 0.04 & 0.04 & 0.03\\
$0.0 < |y_{ee}| < 0.4$ & 0.49 & 0.24 & 0.14 & 1.00 & 0.01 & -0.01 & 0.01 & -0.01 & 0.01 & 0.20 & 0.28 & 0.26 & 0.25 & 0.18 & 0.12\\
$0.4 < |y_{ee}| < 0.8$ & 0.45 & 0.30 & 0.13 & 0.01 & 1.00 & -0.01 & -0.01 & -0.01 & -0.00 & 0.26 & 0.24 & 0.21 & 0.18 & 0.18 & 0.22\\
$0.8 < |y_{ee}| < 1.2$ & 0.38 & 0.24 & 0.06 & -0.01 & -0.01 & 1.00 & 0.00 & -0.00 & -0.00 & 0.24 & 0.15 & 0.17 & 0.22 & 0.15 & 0.16\\
$1.2 < |y_{ee}| < 1.6$ & 0.37 & 0.10 & 0.04 & 0.01 & -0.01 & 0.00 & 1.00 & -0.01 & 0.00 & 0.07 & 0.20 & 0.26 & 0.23 & 0.10 & 0.01\\
$1.6 < |y_{ee}| < 2.0$ & 0.19 & 0.01 & -0.01 & -0.01 & -0.01 & -0.00 & -0.01 & 1.00 & 0.01 & 0.16 & 0.12 & 0.12 & -0.01 & -0.00 & 0.01\\
$2.0 < |y_{ee}| < 2.4$ & 0.08 & 0.00 & -0.00 & 0.01 & -0.00 & -0.00 & 0.00 & 0.01 & 1.00 & 0.16 & 0.02 & -0.00 & -0.00 & -0.01 & 0.00\\
$0.0 < |\Delta \eta_{ee}| < 0.5$ & 0.34 & 0.22 & 0.15 & 0.20 & 0.26 & 0.24 & 0.07 & 0.16 & 0.16 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & -0.00\\
$0.5 < |\Delta \eta_{ee}| < 1.0$ & 0.38 & 0.22 & 0.11 & 0.28 & 0.24 & 0.15 & 0.20 & 0.12 & 0.02 & 0.00 & 1.00 & 0.00 & -0.00 & -0.00 & 0.01\\
$1.0 < |\Delta \eta_{ee}| < 1.5$ & 0.44 & 0.14 & 0.06 & 0.26 & 0.21 & 0.17 & 0.26 & 0.12 & -0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & -0.02\\
$1.5 < |\Delta \eta_{ee}| < 2.0$ & 0.39 & 0.17 & 0.04 & 0.25 & 0.18 & 0.22 & 0.23 & -0.01 & -0.00 & 0.00 & -0.00 & 0.00 & 1.00 & 0.01 & 0.00\\
$2.0 < |\Delta \eta_{ee}| < 2.5$ & 0.26 & 0.15 & 0.04 & 0.18 & 0.18 & 0.15 & 0.10 & -0.00 & -0.01 & 0.00 & -0.00 & 0.00 & 0.01 & 1.00 & -0.00\\
$2.5 < |\Delta \eta_{ee}| < 3.0$ & 0.24 & 0.12 & 0.03 & 0.12 & 0.22 & 0.16 & 0.01 & 0.01 & 0.00 & -0.00 & 0.01 & -0.02 & 0.00 & -0.00 & 1.00\\
\end{tabular} }
\caption{Statistical correlation between the measurement bins in mass, rapidity and $\Delta \eta$ in the electron channel for 500~GeV < \mll\ < 1500~GeV.}
\label{table:elec_corr_500to1500}
\end{center}
\end{sidewaystable}


==> Shared/tables/theory/CombinedTheory_Deta.tex <==
\begin{table}[!htb]
\begin{center}
\resizebox{8cm}{!}{
\begin{tabular}{rc|rr|rrrrr}
\hline\hline
$m_{\ell\ell}$  &  $|\Delta\eta_{\ell\ell}|$  & $\frac{\text{d}^2\sigma}{\text{d}m_{\ell\ell}\text{d}|\Delta\eta_{\ell\ell}|}$  & 
$f^{\rm PI}$           &  
$\delta^{\rm stat}$           &  
$\delta^{\rm pdf}$     &  $\delta^{\rm \alpha_s}$ &  $\delta^{\rm scale}$  &  $\delta^{\rm PI}$   \\
{[\GeV]} & & [pb/\GeV] & [\%] & [\%] & [\%] & [\%] & [\%] & [\%] \\
\hline
$  116 -  150$ & $0.00 - 0.25$ & $4.82 \times 10^{-2}$ &  0.64 &  0.1 & $^{+1.4}_{-1.3}$ &  $^{+0.8}_{-0.9}$ & $^{+0.4}_{-0.5}$ & $^{+0.4}_{-0.4}$  \\  [2pt]
$  116 -  150$ & $0.25 - 0.50$ & $4.58 \times 10^{-2}$ &  0.68 &  0.2 & $^{+1.4}_{-1.3}$ &  $^{+0.8}_{-0.9}$ & $^{+0.5}_{-0.9}$ & $^{+0.4}_{-0.4}$  \\  [2pt]
$  116 -  150$ & $0.50 - 0.75$ & $4.28 \times 10^{-2}$ &  0.74 &  0.2 & $^{+1.4}_{-1.3}$ &  $^{+0.9}_{-0.9}$ & $^{+0.4}_{-0.4}$ & $^{+0.5}_{-0.5}$  \\  [2pt]
$  116 -  150$ & $0.75 - 1.00$ & $3.93 \times 10^{-2}$ &  0.84 &  0.2 & $^{+1.4}_{-1.3}$ &  $^{+0.9}_{-0.9}$ & $^{+0.4}_{-0.9}$ & $^{+0.5}_{-0.5}$  \\  [2pt]
$  116 -  150$ & $1.00 - 1.25$ & $3.53 \times 10^{-2}$ &  0.96 &  0.2 & $^{+1.4}_{-1.3}$ &  $^{+0.9}_{-1.0}$ & $^{+0.1}_{-0.8}$ & $^{+0.6}_{-0.6}$  \\  [2pt]
$  116 -  150$ & $1.25 - 1.50$ & $3.03 \times 10^{-2}$ &  1.15 &  0.2 & $^{+1.5}_{-1.3}$ &  $^{+0.9}_{-0.9}$ & $^{+0.8}_{-0.4}$ & $^{+0.7}_{-0.7}$  \\  [2pt]
$  116 -  150$ & $1.50 - 1.75$ & $2.53 \times 10^{-2}$ &  1.39 &  0.3 & $^{+1.5}_{-1.4}$ &  $^{+0.8}_{-0.9}$ & $^{+0.1}_{-0.6}$ & $^{+0.9}_{-0.9}$  \\  [2pt]
$  116 -  150$ & $1.75 - 2.00$ & $1.96 \times 10^{-2}$ &  1.62 &  0.3 & $^{+1.4}_{-1.3}$ &  $^{+0.9}_{-1.0}$ & $^{+2.3}_{-2.5}$ & $^{+1.0}_{-1.0}$  \\  [2pt]
$  116 -  150$ & $2.00 - 2.25$ & $1.16 \times 10^{-2}$ &  1.49 &  0.2 & $^{+1.3}_{-1.3}$ &  $^{+1.0}_{-1.1}$ & $^{+2.2}_{-3.4}$ & $^{+0.9}_{-0.9}$  \\  [2pt]
$  116 -  150$ & $2.25 - 2.50$ & $4.02 \times 10^{-3}$ &  1.17 &  0.5 & $^{+1.2}_{-1.2}$ &  $^{+1.0}_{-1.1}$ & $^{+3.3}_{-3.5}$ & $^{+0.7}_{-0.7}$  \\  [2pt]
$  116 -  150$ & $2.50 - 2.75$ & $6.54 \times 10^{-4}$ &  0.00 &  0.6 & $^{+1.1}_{-1.2}$ &  $^{+1.0}_{-1.2}$ & $^{+4.9}_{-4.2}$ & $^{+0.0}_{-0.0}$  \\  [2pt]
$  116 -  150$ & $2.75 - 3.00$ & $1.07 \times 10^{-5}$ &  0.00 &  1.3 & $^{+1.0}_{-1.1}$ &  $^{+0.9}_{-1.0}$ & $^{+12.3}_{-9.0}$ & $^{+0.0}_{-0.0}$  \\  [2pt]
\hline
$  150 -  200$ & $0.00 - 0.25$ & $1.05 \times 10^{-2}$ &  1.16 &  0.1 & $^{+1.5}_{-1.6}$ &  $^{+0.8}_{-0.8}$ & $^{+0.5}_{-0.4}$ & $^{+0.7}_{-0.7}$  \\  [2pt]
$  150 -  200$ & $0.25 - 0.50$ & $1.00 \times 10^{-2}$ &  1.23 &  0.2 & $^{+1.5}_{-1.6}$ &  $^{+0.8}_{-0.8}$ & $^{+0.2}_{-0.6}$ & $^{+0.8}_{-0.8}$  \\  [2pt]
$  150 -  200$ & $0.50 - 0.75$ & $9.44 \times 10^{-3}$ &  1.33 &  0.2 & $^{+1.5}_{-1.6}$ &  $^{+0.8}_{-0.8}$ & $^{+0.2}_{-0.9}$ & $^{+0.8}_{-0.8}$  \\  [2pt]
$  150 -  200$ & $0.75 - 1.00$ & $8.69 \times 10^{-3}$ &  1.50 &  0.2 & $^{+1.5}_{-1.6}$ &  $^{+0.8}_{-0.8}$ & $^{+0.7}_{+0.0}$ & $^{+0.9}_{-0.9}$  \\  [2pt]
$  150 -  200$ & $1.00 - 1.25$ & $7.86 \times 10^{-3}$ &  1.73 &  0.2 & $^{+1.5}_{-1.6}$ &  $^{+0.8}_{-0.8}$ & $^{+0.6}_{-0.6}$ & $^{+1.1}_{-1.1}$  \\  [2pt]
$  150 -  200$ & $1.25 - 1.50$ & $6.86 \times 10^{-3}$ &  2.04 &  0.2 & $^{+1.5}_{-1.6}$ &  $^{+0.8}_{-0.8}$ & $^{+0.5}_{-0.7}$ & $^{+1.3}_{-1.3}$  \\  [2pt]
$  150 -  200$ & $1.50 - 1.75$ & $5.82 \times 10^{-3}$ &  2.45 &  0.2 & $^{+1.5}_{-1.6}$ &  $^{+0.8}_{-0.8}$ & $^{-0.1}_{-0.6}$ & $^{+1.5}_{-1.5}$  \\  [2pt]
$  150 -  200$ & $1.75 - 2.00$ & $4.77 \times 10^{-3}$ &  3.01 &  0.3 & $^{+1.5}_{-1.6}$ &  $^{+0.8}_{-0.8}$ & $^{+0.4}_{-0.5}$ & $^{+1.9}_{-1.9}$  \\  [2pt]
$  150 -  200$ & $2.00 - 2.25$ & $3.76 \times 10^{-3}$ &  3.77 &  0.3 & $^{+1.5}_{-1.5}$ &  $^{+0.8}_{-0.8}$ & $^{+0.4}_{-0.5}$ & $^{+2.4}_{-2.4}$  \\  [2pt]
$  150 -  200$ & $2.25 - 2.50$ & $2.86 \times 10^{-3}$ &  4.82 &  0.3 & $^{+1.5}_{-1.5}$ &  $^{+0.8}_{-0.8}$ & $^{+0.4}_{-0.7}$ & $^{+3.1}_{-3.1}$  \\  [2pt]
$  150 -  200$ & $2.50 - 2.75$ & $1.93 \times 10^{-3}$ &  5.00 &  0.3 & $^{+1.4}_{-1.5}$ &  $^{+0.8}_{-0.9}$ & $^{+1.9}_{-3.4}$ & $^{+3.2}_{-3.2}$  \\  [2pt]
$  150 -  200$ & $2.75 - 3.00$ & $8.52 \times 10^{-4}$ &  4.79 &  0.5 & $^{+1.4}_{-1.4}$ &  $^{+0.9}_{-0.9}$ & $^{+3.1}_{-4.4}$ & $^{+3.1}_{-3.1}$  \\  [2pt]
\hline
$  200 -  300$ & $0.00 - 0.25$ & $2.18 \times 10^{-3}$ &  1.65 &  0.1 & $^{+1.7}_{-1.9}$ &  $^{+0.6}_{-0.6}$ & $^{+0.7}_{-0.2}$ & $^{+1.0}_{-1.0}$  \\  [2pt]
$  200 -  300$ & $0.25 - 0.50$ & $2.11 \times 10^{-3}$ &  1.72 &  0.2 & $^{+1.7}_{-1.9}$ &  $^{+0.6}_{-0.6}$ & $^{+0.6}_{-0.4}$ & $^{+1.1}_{-1.1}$  \\  [2pt]
$  200 -  300$ & $0.50 - 0.75$ & $2.00 \times 10^{-3}$ &  1.88 &  0.2 & $^{+1.7}_{-1.9}$ &  $^{+0.6}_{-0.7}$ & $^{+0.3}_{-0.6}$ & $^{+1.2}_{-1.2}$  \\  [2pt]
$  200 -  300$ & $0.75 - 1.00$ & $1.87 \times 10^{-3}$ &  2.10 &  0.2 & $^{+1.7}_{-1.9}$ &  $^{+0.7}_{-0.7}$ & $^{+0.2}_{-0.8}$ & $^{+1.3}_{-1.3}$  \\  [2pt]
$  200 -  300$ & $1.00 - 1.25$ & $1.69 \times 10^{-3}$ &  2.42 &  0.2 & $^{+1.7}_{-1.9}$ &  $^{+0.7}_{-0.7}$ & $^{+0.4}_{-0.2}$ & $^{+1.5}_{-1.5}$  \\  [2pt]
$  200 -  300$ & $1.25 - 1.50$ & $1.49 \times 10^{-3}$ &  2.86 &  0.2 & $^{+1.7}_{-1.9}$ &  $^{+0.7}_{-0.7}$ & $^{+0.4}_{-0.6}$ & $^{+1.8}_{-1.8}$  \\  [2pt]
$  200 -  300$ & $1.50 - 1.75$ & $1.27 \times 10^{-3}$ &  3.43 &  0.2 & $^{+1.7}_{-1.8}$ &  $^{+0.7}_{-0.7}$ & $^{+0.6}_{-0.3}$ & $^{+2.2}_{-2.2}$  \\  [2pt]
$  200 -  300$ & $1.75 - 2.00$ & $1.07 \times 10^{-3}$ &  4.15 &  0.3 & $^{+1.7}_{-1.8}$ &  $^{+0.7}_{-0.7}$ & $^{+0.2}_{-1.0}$ & $^{+2.6}_{-2.6}$  \\  [2pt]
$  200 -  300$ & $2.00 - 2.25$ & $8.51 \times 10^{-4}$ &  5.17 &  0.3 & $^{+1.7}_{-1.8}$ &  $^{+0.6}_{-0.7}$ & $^{+0.6}_{+0.0}$ & $^{+3.3}_{-3.3}$  \\  [2pt]
$  200 -  300$ & $2.25 - 2.50$ & $6.70 \times 10^{-4}$ &  6.42 &  0.3 & $^{+1.7}_{-1.8}$ &  $^{+0.6}_{-0.7}$ & $^{+0.5}_{-0.6}$ & $^{+4.1}_{-4.1}$  \\  [2pt]
$  200 -  300$ & $2.50 - 2.75$ & $5.09 \times 10^{-4}$ &  8.09 &  0.4 & $^{+1.7}_{-1.8}$ &  $^{+0.6}_{-0.7}$ & $^{+0.9}_{-0.3}$ & $^{+5.2}_{-5.2}$  \\  [2pt]
$  200 -  300$ & $2.75 - 3.00$ & $3.76 \times 10^{-4}$ & 10.35 &  0.5 & $^{+1.7}_{-1.7}$ &  $^{+0.6}_{-0.6}$ & $^{+0.4}_{-0.6}$ & $^{+6.7}_{-6.7}$  \\  [2pt]
\hline
$  300 -  500$ & $0.00 - 0.50$ & $2.84 \times 10^{-4}$ &  2.36 &  0.0 & $^{+2.1}_{-2.3}$ &  $^{+0.4}_{-0.4}$ & $^{+0.4}_{-0.4}$ & $^{+1.5}_{-1.5}$  \\  [2pt]
$  300 -  500$ & $0.50 - 1.00$ & $2.64 \times 10^{-4}$ &  2.72 &  0.1 & $^{+2.1}_{-2.3}$ &  $^{+0.5}_{-0.4}$ & $^{+0.4}_{-0.7}$ & $^{+1.8}_{-1.8}$  \\  [2pt]
$  300 -  500$ & $1.00 - 1.50$ & $2.25 \times 10^{-4}$ &  3.53 &  0.1 & $^{+2.1}_{-2.3}$ &  $^{+0.5}_{-0.4}$ & $^{+0.2}_{-0.3}$ & $^{+2.3}_{-2.3}$  \\  [2pt]
$  300 -  500$ & $1.50 - 2.00$ & $1.69 \times 10^{-4}$ &  5.03 &  0.1 & $^{+2.1}_{-2.3}$ &  $^{+0.5}_{-0.5}$ & $^{+0.5}_{-0.3}$ & $^{+3.3}_{-3.3}$  \\  [2pt]
$  300 -  500$ & $2.00 - 2.50$ & $1.14 \times 10^{-4}$ &  7.55 &  0.1 & $^{+2.1}_{-2.2}$ &  $^{+0.5}_{-0.5}$ & $^{+0.3}_{-0.4}$ & $^{+4.9}_{-4.9}$  \\  [2pt]
$  300 -  500$ & $2.50 - 3.00$ & $6.88 \times 10^{-5}$ & 11.69 &  0.2 & $^{+2.0}_{-2.1}$ &  $^{+0.5}_{-0.5}$ & $^{+0.5}_{-0.3}$ & $^{+7.7}_{-7.7}$  \\  [2pt]
\hline
$  500 - 1500$ & $0.00 - 0.50$ & $9.08 \times 10^{-6}$ &  3.77 &  0.0 & $^{+2.6}_{-2.9}$ &  $^{+0.2}_{-0.1}$ & $^{+0.5}_{-0.5}$ & $^{+2.7}_{-2.7}$  \\  [2pt]
$  500 - 1500$ & $0.50 - 1.00$ & $8.83 \times 10^{-6}$ &  4.23 &  0.1 & $^{+2.6}_{-2.9}$ &  $^{+0.2}_{-0.1}$ & $^{+0.3}_{-0.5}$ & $^{+3.0}_{-3.0}$  \\  [2pt]
$  500 - 1500$ & $1.00 - 1.50$ & $7.92 \times 10^{-6}$ &  5.30 &  0.1 & $^{+2.6}_{-2.9}$ &  $^{+0.2}_{-0.1}$ & $^{+0.5}_{-0.6}$ & $^{+3.7}_{-3.7}$  \\  [2pt]
$  500 - 1500$ & $1.50 - 2.00$ & $6.34 \times 10^{-6}$ &  7.25 &  0.1 & $^{+2.6}_{-2.9}$ &  $^{+0.2}_{-0.1}$ & $^{+0.4}_{-0.4}$ & $^{+5.0}_{-5.0}$  \\  [2pt]
$  500 - 1500$ & $2.00 - 2.50$ & $4.50 \times 10^{-6}$ & 10.55 &  0.1 & $^{+2.5}_{-2.8}$ &  $^{+0.2}_{-0.1}$ & $^{+0.3}_{-0.4}$ & $^{+7.3}_{-7.3}$  \\  [2pt]
$  500 - 1500$ & $2.50 - 3.00$ & $2.88 \times 10^{-6}$ & 15.96 &  0.1 & $^{+2.4}_{-2.7}$ &  $^{+0.2}_{-0.1}$ & $^{+0.2}_{-0.6}$ & $^{+11.1}_{-11.1}$  \\  [2pt]
\hline
\hline
\end{tabular}   } %end resizebox
\caption{Born-level differential fiducial cross section $\frac{\text{d}\sigma}{\text{d}m_{\ell\ell}\text{d}|\Delta\eta_{\ell\ell}|}$
at NNLO including NLO electroweak corrections and the PI contribution. The fraction of the PI contribution, $f^{\rm PI}$, is also given.
The calculation is performed using the MMHT NNLO PDF set and with dynamic scales $\mu_r=\mu_f=m_{\ell\ell}$.
The predictions are listed together with the statistical uncertainty ($\delta^{\rm stat}$),
the PDF eigenvector variation ($\delta^{\rm pdf}$), the uncertainty from the variation of $\alpha_s$, $\mu_F$ and $\mu_R$ ($\delta^{\rm \alpha_s}$, $\delta^{\rm scale}$),
and the uncertainty from the variation of the photon PDF in the PI contribution ($\delta^{\rm PI}$).}
\label{table:TheoryXsec_Deta}
\end{center}
\end{table}


==> Shared/tables/theory/CombinedTheory_M.tex <==
\begin{table}[!htb]
\begin{center}
\resizebox{8cm}{!}{
\begin{tabular}{r|rr|rrrrr}
\hline\hline
$m_{\ell\ell}$  &  $\frac{\text{d}\sigma}{\text{d}m_{\ell\ell}}$  & 
$f^{\rm PI}$           &  
$\delta^{\rm stat}$           &  
$\delta^{\rm pdf}$     &  $\delta^{\rm \alpha_s}$ &  $\delta^{\rm scale}$   &  $\delta^{\rm PI}$    \\
{[\GeV]} & [pb/\GeV] & [\%] & [\%] & [\%] & [\%] & [\%] & [\%] \\
\hline
$  116 -  130$ & $2.22 \times 10^{-1}$ & $ 0.74$ & $ 0.0$ & $^{+1.4}_{-1.3}$ &  $^{+0.9}_{-1.0}$ &  $^{+0.5}_{-0.7}$ &  $^{+0.5}_{-0.5}$    \\ [2pt]
$  130 -  150$ & $1.02 \times 10^{-1}$ & $ 1.24$ & $ 0.0$ & $^{+1.4}_{-1.4}$ &  $^{+0.8}_{-0.9}$ &  $^{+0.5}_{-0.6}$ &  $^{+0.8}_{-0.8}$    \\ [2pt]
$  150 -  175$ & $4.84 \times 10^{-2}$ & $ 1.82$ & $ 0.0$ & $^{+1.5}_{-1.5}$ &  $^{+0.8}_{-0.8}$ &  $^{+0.4}_{-0.5}$ &  $^{+1.1}_{-1.1}$    \\ [2pt]
$  175 -  200$ & $2.51 \times 10^{-2}$ & $ 2.40$ & $ 0.0$ & $^{+1.6}_{-1.6}$ &  $^{+0.7}_{-0.8}$ &  $^{+0.3}_{-0.5}$ &  $^{+1.5}_{-1.5}$    \\ [2pt]
$  200 -  230$ & $1.38 \times 10^{-2}$ & $ 2.95$ & $ 0.0$ & $^{+1.6}_{-1.8}$ &  $^{+0.7}_{-0.7}$ &  $^{+0.3}_{-0.3}$ &  $^{+1.9}_{-1.9}$    \\ [2pt]
$  230 -  260$ & $7.87 \times 10^{-3}$ & $ 3.48$ & $ 0.0$ & $^{+1.7}_{-1.9}$ &  $^{+0.6}_{-0.6}$ &  $^{+0.3}_{-0.3}$ &  $^{+2.2}_{-2.2}$    \\ [2pt]
$  260 -  300$ & $4.47 \times 10^{-3}$ & $ 4.03$ & $ 0.0$ & $^{+1.8}_{-2.0}$ &  $^{+0.6}_{-0.6}$ &  $^{+0.2}_{-0.3}$ &  $^{+2.6}_{-2.6}$    \\ [2pt]
$  300 -  380$ & $2.00 \times 10^{-3}$ & $ 4.82$ & $ 0.0$ & $^{+2.0}_{-2.2}$ &  $^{+0.5}_{-0.5}$ &  $^{+0.3}_{-0.4}$ &  $^{+3.1}_{-3.1}$    \\ [2pt]
$  380 -  500$ & $6.51 \times 10^{-4}$ & $ 5.95$ & $ 0.0$ & $^{+2.2}_{-2.4}$ &  $^{+0.4}_{-0.3}$ &  $^{+0.3}_{-0.4}$ &  $^{+4.0}_{-4.0}$    \\ [2pt]
$  500 -  700$ & $1.61 \times 10^{-4}$ & $ 7.48$ & $ 0.0$ & $^{+2.5}_{-2.7}$ &  $^{+0.2}_{-0.2}$ &  $^{+0.4}_{-0.5}$ &  $^{+5.1}_{-5.1}$    \\ [2pt]
$  700 - 1000$ & $2.90 \times 10^{-5}$ & $10.02$ & $ 0.0$ & $^{+2.8}_{-3.1}$ &  $^{+0.1}_{-0.0}$ &  $^{+0.4}_{-0.5}$ &  $^{+7.1}_{-7.1}$    \\ [2pt]
$ 1000 - 1500$ & $3.64 \times 10^{-6}$ & $14.83$ & $ 0.1$ & $^{+3.1}_{-3.3}$ &  $^{+0.3}_{-0.2}$ &  $^{+0.5}_{-0.6}$ &  $^{+11.2}_{-11.2}$    \\ [2pt]
\hline
\hline
\end{tabular}  } %end resizebox
\caption{Born-level differential fiducial cross section $\frac{\text{d}\sigma}{\text{d}m_{\ell\ell}}$ at NNLO including NLO electroweak corrections 
and the PI contribution. The fraction of the PI contribution, $f^{\rm PI}$, is also given.
The calculation is performed using the MMHT NNLO PDF set and with dynamic scales $\mu_r=\mu_f=m_{\ell\ell}$.
The predictions are listed together with the statistical uncertainty ($\delta^{\rm stat}$),
the PDF eigenvector variation ($\delta^{\rm pdf}$), the uncertainty from the variation of $\alpha_s$, $\mu_F$ and $\mu_R$ ($\delta^{\rm \alpha_s}$, $\delta^{\rm scale}$),
and the uncertainty from the variation of the photon PDF in the PI contribution ($\delta^{\rm PI}$).}
\label{table:TheoryXsec_Mass}
\end{center}
\end{table}


==> Shared/tables/theory/CombinedTheory_y.tex <==
\begin{table}[!htb]
\begin{center}
\resizebox{8cm}{!}{
\begin{tabular}{rc|rr|rrrrr}
\hline\hline
$m_{\ell\ell}$  &  $|y_{\ell\ell}|$  & $\frac{\text{d}^2\sigma}{\text{d}m_{\ell\ell}\text{d}|y_{\ell\ell}|}$  & 
$f^{\rm PI}$           &  
$\delta^{\rm stat}$           &  
$\delta^{\rm pdf}$     &  $\delta^{\rm \alpha_s}$ &  $\delta^{\rm scale}$   &  $\delta^{\rm PI}$   \\
{[\GeV]} & & [pb/\GeV] & [\%] & [\%] & [\%] & [\%] & [\%] & [\%] \\
\hline
$  116 -  150$ & $ 0.0 -  0.2$ & $3.92 \times 10^{-2}$ &  1.12 &  0.1 & $^{+1.5}_{-1.4}$ &  $^{+0.9}_{-0.9}$ &  $^{+0.6}_{-0.5}$ & $^{+0.7}_{-0.7}$   \\ [2pt]
$  116 -  150$ & $ 0.2 -  0.4$ & $3.92 \times 10^{-2}$ &  1.10 &  0.1 & $^{+1.5}_{-1.4}$ &  $^{+0.9}_{-1.0}$ &  $^{+0.6}_{-0.6}$ & $^{+0.7}_{-0.7}$   \\ [2pt]
$  116 -  150$ & $ 0.4 -  0.6$ & $3.91 \times 10^{-2}$ &  1.08 &  0.1 & $^{+1.4}_{-1.4}$ &  $^{+0.9}_{-1.0}$ &  $^{+0.5}_{-0.8}$ & $^{+0.7}_{-0.7}$   \\ [2pt]
$  116 -  150$ & $ 0.6 -  0.8$ & $3.89 \times 10^{-2}$ &  1.06 &  0.1 & $^{+1.4}_{-1.3}$ &  $^{+0.9}_{-1.0}$ &  $^{+0.5}_{-0.6}$ & $^{+0.7}_{-0.7}$   \\ [2pt]
$  116 -  150$ & $ 0.8 -  1.0$ & $3.88 \times 10^{-2}$ &  1.02 &  0.1 & $^{+1.4}_{-1.3}$ &  $^{+0.9}_{-1.0}$ &  $^{+0.4}_{-1.0}$ & $^{+0.6}_{-0.6}$   \\ [2pt]
$  116 -  150$ & $ 1.0 -  1.2$ & $3.83 \times 10^{-2}$ &  0.98 &  0.1 & $^{+1.5}_{-1.4}$ &  $^{+0.9}_{-1.0}$ &  $^{+0.5}_{-0.4}$ & $^{+0.6}_{-0.6}$   \\ [2pt]
$  116 -  150$ & $ 1.2 -  1.4$ & $3.73 \times 10^{-2}$ &  0.94 &  0.1 & $^{+1.5}_{-1.4}$ &  $^{+0.9}_{-1.0}$ &  $^{+0.7}_{-0.8}$ & $^{+0.6}_{-0.6}$   \\ [2pt]
$  116 -  150$ & $ 1.4 -  1.6$ & $3.44 \times 10^{-2}$ &  0.85 &  0.1 & $^{+1.5}_{-1.5}$ &  $^{+0.9}_{-1.0}$ &  $^{+0.5}_{-0.7}$ & $^{+0.5}_{-0.5}$   \\ [2pt]
$  116 -  150$ & $ 1.6 -  1.8$ & $2.89 \times 10^{-2}$ &  0.71 &  0.1 & $^{+1.6}_{-1.5}$ &  $^{+0.9}_{-0.9}$ &  $^{+0.7}_{-0.8}$ & $^{+0.4}_{-0.4}$   \\ [2pt]
$  116 -  150$ & $ 1.8 -  2.0$ & $2.22 \times 10^{-2}$ &  0.58 &  0.2 & $^{+1.6}_{-1.6}$ &  $^{+0.9}_{-0.9}$ &  $^{+0.5}_{-0.7}$ & $^{+0.4}_{-0.4}$   \\ [2pt]
$  116 -  150$ & $ 2.0 -  2.2$ & $1.47 \times 10^{-2}$ &  0.49 &  0.2 & $^{+1.7}_{-1.7}$ &  $^{+0.8}_{-0.9}$ &  $^{+0.6}_{-0.4}$ & $^{+0.3}_{-0.3}$   \\ [2pt]
$  116 -  150$ & $ 2.2 -  2.4$ & $7.10 \times 10^{-3}$ &  0.42 &  0.3 & $^{+1.8}_{-1.8}$ &  $^{+0.8}_{-0.8}$ &  $^{+0.0}_{-1.8}$ & $^{+0.3}_{-0.3}$   \\ [2pt]
\hline
$  150 -  200$ & $ 0.0 -  0.2$ & $1.00 \times 10^{-2}$ &  2.57 &  0.1 & $^{+1.5}_{-1.6}$ &  $^{+0.8}_{-0.8}$ &  $^{+0.3}_{-0.5}$ & $^{+1.6}_{-1.6}$   \\ [2pt]
$  150 -  200$ & $ 0.2 -  0.4$ & $1.00 \times 10^{-2}$ &  2.53 &  0.1 & $^{+1.5}_{-1.5}$ &  $^{+0.8}_{-0.8}$ &  $^{+0.5}_{-0.5}$ & $^{+1.6}_{-1.6}$   \\ [2pt]
$  150 -  200$ & $ 0.4 -  0.6$ & $1.00 \times 10^{-2}$ &  2.47 &  0.1 & $^{+1.5}_{-1.5}$ &  $^{+0.8}_{-0.8}$ &  $^{+0.1}_{-0.7}$ & $^{+1.6}_{-1.6}$   \\ [2pt]
$  150 -  200$ & $ 0.6 -  0.8$ & $9.95 \times 10^{-3}$ &  2.39 &  0.1 & $^{+1.5}_{-1.5}$ &  $^{+0.8}_{-0.8}$ &  $^{+0.6}_{-0.3}$ & $^{+1.5}_{-1.5}$   \\ [2pt]
$  150 -  200$ & $ 0.8 -  1.0$ & $9.86 \times 10^{-3}$ &  2.29 &  0.1 & $^{+1.5}_{-1.6}$ &  $^{+0.8}_{-0.8}$ &  $^{+0.3}_{-0.4}$ & $^{+1.4}_{-1.4}$   \\ [2pt]
$  150 -  200$ & $ 1.0 -  1.2$ & $9.52 \times 10^{-3}$ &  2.13 &  0.1 & $^{+1.5}_{-1.6}$ &  $^{+0.8}_{-0.8}$ &  $^{+0.4}_{-0.5}$ & $^{+1.3}_{-1.3}$   \\ [2pt]
$  150 -  200$ & $ 1.2 -  1.4$ & $8.82 \times 10^{-3}$ &  1.81 &  0.1 & $^{+1.6}_{-1.7}$ &  $^{+0.8}_{-0.8}$ &  $^{+0.3}_{-0.7}$ & $^{+1.1}_{-1.1}$   \\ [2pt]
$  150 -  200$ & $ 1.4 -  1.6$ & $7.74 \times 10^{-3}$ &  1.47 &  0.1 & $^{+1.6}_{-1.7}$ &  $^{+0.8}_{-0.8}$ &  $^{+0.7}_{-0.3}$ & $^{+0.9}_{-0.9}$   \\ [2pt]
$  150 -  200$ & $ 1.6 -  1.8$ & $6.42 \times 10^{-3}$ &  1.19 &  0.1 & $^{+1.7}_{-1.8}$ &  $^{+0.8}_{-0.8}$ &  $^{+0.6}_{-0.6}$ & $^{+0.7}_{-0.7}$   \\ [2pt]
$  150 -  200$ & $ 1.8 -  2.0$ & $4.85 \times 10^{-3}$ &  0.96 &  0.1 & $^{+1.7}_{-1.9}$ &  $^{+0.8}_{-0.8}$ &  $^{+0.4}_{-0.7}$ & $^{+0.6}_{-0.6}$   \\ [2pt]
$  150 -  200$ & $ 2.0 -  2.2$ & $3.13 \times 10^{-3}$ &  0.79 &  0.2 & $^{+1.8}_{-2.0}$ &  $^{+0.7}_{-0.7}$ &  $^{+0.1}_{-0.7}$ & $^{+0.5}_{-0.5}$   \\ [2pt]
$  150 -  200$ & $ 2.2 -  2.4$ & $1.44 \times 10^{-3}$ &  0.68 &  0.3 & $^{+1.9}_{-2.1}$ &  $^{+0.7}_{-0.6}$ &  $^{+1.3}_{-0.1}$ & $^{+0.4}_{-0.4}$   \\ [2pt]
\hline
$  200 -  300$ & $ 0.0 -  0.2$ & $2.42 \times 10^{-3}$ &  4.66 &  0.1 & $^{+1.8}_{-1.9}$ &  $^{+0.6}_{-0.7}$ &  $^{+0.2}_{-0.4}$ & $^{+3.0}_{-3.0}$   \\ [2pt]
$  200 -  300$ & $ 0.2 -  0.4$ & $2.41 \times 10^{-3}$ &  4.59 &  0.1 & $^{+1.8}_{-1.8}$ &  $^{+0.6}_{-0.7}$ &  $^{+0.3}_{-0.2}$ & $^{+3.0}_{-3.0}$   \\ [2pt]
$  200 -  300$ & $ 0.4 -  0.6$ & $2.40 \times 10^{-3}$ &  4.43 &  0.1 & $^{+1.8}_{-1.8}$ &  $^{+0.6}_{-0.7}$ &  $^{+0.4}_{-0.4}$ & $^{+2.9}_{-2.9}$   \\ [2pt]
$  200 -  300$ & $ 0.6 -  0.8$ & $2.36 \times 10^{-3}$ &  4.16 &  0.1 & $^{+1.7}_{-1.8}$ &  $^{+0.7}_{-0.7}$ &  $^{+0.2}_{-0.5}$ & $^{+2.7}_{-2.7}$   \\ [2pt]
$  200 -  300$ & $ 0.8 -  1.0$ & $2.26 \times 10^{-3}$ &  3.67 &  0.1 & $^{+1.7}_{-1.8}$ &  $^{+0.7}_{-0.7}$ &  $^{+0.4}_{-0.2}$ & $^{+2.3}_{-2.3}$   \\ [2pt]
$  200 -  300$ & $ 1.0 -  1.2$ & $2.12 \times 10^{-3}$ &  2.99 &  0.1 & $^{+1.7}_{-1.9}$ &  $^{+0.7}_{-0.7}$ &  $^{+0.4}_{-0.3}$ & $^{+1.9}_{-1.9}$   \\ [2pt]
$  200 -  300$ & $ 1.2 -  1.4$ & $1.93 \times 10^{-3}$ &  2.38 &  0.1 & $^{+1.7}_{-1.9}$ &  $^{+0.7}_{-0.7}$ &  $^{+0.2}_{-0.4}$ & $^{+1.5}_{-1.5}$   \\ [2pt]
$  200 -  300$ & $ 1.4 -  1.6$ & $1.66 \times 10^{-3}$ &  1.89 &  0.1 & $^{+1.8}_{-2.0}$ &  $^{+0.7}_{-0.6}$ &  $^{+0.6}_{-0.3}$ & $^{+1.2}_{-1.2}$   \\ [2pt]
$  200 -  300$ & $ 1.6 -  1.8$ & $1.35 \times 10^{-3}$ &  1.51 &  0.1 & $^{+1.9}_{-2.1}$ &  $^{+0.6}_{-0.6}$ &  $^{+0.4}_{-0.5}$ & $^{+0.9}_{-0.9}$   \\ [2pt]
$  200 -  300$ & $ 1.8 -  2.0$ & $9.78 \times 10^{-4}$ &  1.20 &  0.1 & $^{+1.9}_{-2.2}$ &  $^{+0.6}_{-0.5}$ &  $^{+0.4}_{-0.6}$ & $^{+0.7}_{-0.7}$   \\ [2pt]
$  200 -  300$ & $ 2.0 -  2.2$ & $5.94 \times 10^{-4}$ &  1.01 &  0.2 & $^{+2.0}_{-2.3}$ &  $^{+0.5}_{-0.5}$ &  $^{+0.5}_{-0.4}$ & $^{+0.6}_{-0.6}$   \\ [2pt]
$  200 -  300$ & $ 2.2 -  2.4$ & $2.52 \times 10^{-4}$ &  0.88 &  0.3 & $^{+2.1}_{-2.4}$ &  $^{+0.5}_{-0.4}$ &  $^{+0.6}_{-0.3}$ & $^{+0.6}_{-0.6}$   \\ [2pt]
\hline
$  300 -  500$ & $ 0.0 -  0.4$ & $3.83 \times 10^{-4}$ &  8.06 &  0.0 & $^{+2.3}_{-2.3}$ &  $^{+0.5}_{-0.5}$ &  $^{+0.1}_{-0.4}$ & $^{+5.4}_{-5.4}$   \\ [2pt]
$  300 -  500$ & $ 0.4 -  0.8$ & $3.63 \times 10^{-4}$ &  6.42 &  0.0 & $^{+2.2}_{-2.3}$ &  $^{+0.5}_{-0.5}$ &  $^{+0.5}_{-0.3}$ & $^{+4.2}_{-4.2}$   \\ [2pt]
$  300 -  500$ & $ 0.8 -  1.2$ & $3.21 \times 10^{-4}$ &  4.25 &  0.0 & $^{+2.0}_{-2.3}$ &  $^{+0.5}_{-0.5}$ &  $^{+0.2}_{-0.5}$ & $^{+2.7}_{-2.7}$   \\ [2pt]
$  300 -  500$ & $ 1.2 -  1.6$ & $2.46 \times 10^{-4}$ &  2.63 &  0.0 & $^{+2.0}_{-2.3}$ &  $^{+0.4}_{-0.4}$ &  $^{+0.4}_{-0.4}$ & $^{+1.6}_{-1.6}$   \\ [2pt]
$  300 -  500$ & $ 1.6 -  2.0$ & $1.37 \times 10^{-4}$ &  1.71 &  0.1 & $^{+2.1}_{-2.5}$ &  $^{+0.4}_{-0.3}$ &  $^{+0.3}_{-0.5}$ & $^{+1.1}_{-1.1}$   \\ [2pt]
$  300 -  500$ & $ 2.0 -  2.4$ & $3.67 \times 10^{-5}$ &  1.52 &  0.1 & $^{+2.2}_{-2.5}$ &  $^{+0.2}_{-0.2}$ &  $^{+0.6}_{-0.4}$ & $^{+1.1}_{-1.1}$   \\ [2pt]
\hline
$  500 - 1500$ & $ 0.0 -  0.4$ & $1.67 \times 10^{-5}$ & 12.58 &  0.0 & $^{+2.7}_{-3.0}$ &  $^{+0.2}_{-0.2}$ &  $^{+0.4}_{-0.4}$ & $^{+8.9}_{-8.9}$   \\ [2pt]
$  500 - 1500$ & $ 0.4 -  0.8$ & $1.50 \times 10^{-5}$ &  8.81 &  0.0 & $^{+2.6}_{-2.9}$ &  $^{+0.2}_{-0.1}$ &  $^{+0.3}_{-0.5}$ & $^{+6.1}_{-6.1}$   \\ [2pt]
$  500 - 1500$ & $ 0.8 -  1.2$ & $1.19 \times 10^{-5}$ &  5.50 &  0.0 & $^{+2.6}_{-2.9}$ &  $^{+0.2}_{-0.0}$ &  $^{+0.4}_{-0.5}$ & $^{+3.6}_{-3.6}$   \\ [2pt]
$  500 - 1500$ & $ 1.2 -  1.6$ & $7.13 \times 10^{-6}$ &  3.68 &  0.0 & $^{+2.6}_{-2.8}$ &  $^{+0.1}_{-0.0}$ &  $^{+0.5}_{-0.5}$ & $^{+2.5}_{-2.5}$   \\ [2pt]
$  500 - 1500$ & $ 1.6 -  2.0$ & $2.46 \times 10^{-6}$ &  3.48 &  0.1 & $^{+2.5}_{-2.7}$ &  $^{+0.1}_{-0.0}$ &  $^{+0.3}_{-0.5}$ & $^{+2.8}_{-2.8}$   \\ [2pt]
$  500 - 1500$ & $ 2.0 -  2.4$ & $2.76 \times 10^{-7}$ &  6.11 &  0.3 & $^{+2.8}_{-2.7}$ &  $^{+0.3}_{-0.1}$ &  $^{+0.9}_{-0.6}$ & $^{+5.6}_{-5.6}$   \\ [2pt]
\hline
\hline
\end{tabular}   }  %end resizebox
\caption{Born-level differential fiducial cross section $\frac{\text{d}^2\sigma}{\text{d}m_{\ell\ell}\text{d}|y_{\ell\ell}|}$
at NNLO including NLO electroweak corrections and the PI contribution. The fraction of the PI contribution, $f^{\rm PI}$, is also given.
The calculation is performed using the MMHT NNLO PDF set and with dynamic scales $\mu_r=\mu_f=m_{\ell\ell}$.
The predictions are listed together with the statistical uncertainty ($\delta^{\rm stat}$),
the PDF eigenvector variation ($\delta^{\rm pdf}$), the uncertainty from the variation of $\alpha_s$, $\mu_F$ and $\mu_R$ ($\delta^{\rm \alpha_s}$, $\delta^{\rm scale}$),
and the uncertainty from the variation of the photon PDF in the PI contribution ($\delta^{\rm PI}$).}
\label{table:TheoryXsec_Rapidity}
\end{center}
\end{table}


==> Shared/tables/theory/chi2.tex <==
\begin{table}[!htb]
\begin{center}
%\resizebox{0.5\textwidth}{!}{
\begin{tabular}{r|rrr}
\hline
	PDF   & $m_{\ell\ell}$ & $|y_{\ell\ell}|$ & $|\Delta \eta_{\ell\ell}|$ \\
\hline
 MMHT2014  & 19.5/12  & 63.1/48  & 68.8/47	 \\
 CT14 	     & 17.1/12  & 53.5/48  & 67.5/47	 \\
 NNPDF3.0     & 21.2/12  & 64.7/48  & 69.3/47        \\
 HERAPDF2.0 & 15.6/12  & 60.9/48  & 68.5/47       \\
 ABM12	     & 14.4/12  & 58.4/48  & 55.1/47	\\
\hline
\end{tabular} 
%}%end of resizebox
\caption{The $\chi^2/dof$ values for the compatibility of data and
  theory after the minimization procedure using five different PDF sets.}
\label{table:chi2}
\end{center}
\end{table}

